Unsupervised Multi-Index Semantic Hashing

Semantic hashing represents documents as compact binary vectors (hash codes) and allows both efficient and effective similarity search in large-scale information retrieval. The state of the art has primarily focused on learning hash codes that improve similarity search effectiveness, while assuming a brute-force linear scan strategy for searching over all the hash codes, even though much faster alternatives exist. One such alternative is multi-index hashing, an approach that constructs a smaller candidate set to search over, which depending on the distribution of the hash codes can lead to sub-linear search time. In this work, we propose Multi-Index Semantic Hashing (MISH), an unsupervised hashing model that learns hash codes that are both effective and highly efficient by being optimized for multi-index hashing. We derive novel training objectives, which enable to learn hash codes that reduce the candidate sets produced by multi-index hashing, while being end-to-end trainable. In fact, our proposed training objectives are model agnostic, i.e., not tied to how the hash codes are generated specifically in MISH, and are straight-forward to include in existing and future semantic hashing models. We experimentally compare MISH to state-of-the-art semantic hashing baselines in the task of document similarity search. We find that even though multi-index hashing also improves the efficiency of the baselines compared to a linear scan, they are still upwards of 33% slower than MISH, while MISH is still able to obtain state-of-the-art effectiveness.

==> Unsupervised Multi-Index Semantic Hashing (WWW) (1)/deltatable.tex <==
\begin{table}
    \centering
    \resizebox{\linewidth}{!}
    {
    \begin{tabular}{l|cc|cc}
    \toprule
    & \multicolumn{2}{c}{32 bits} & \multicolumn{2}{c}{64 bits} \\ 
    & $\Delta$ worst case & $\Delta$ average & $\Delta$ worst case & $\Delta$ average \\ \midrule
LCH & -16.65\% & -12.57\% & -12.93\% & -11.46\% \\
STH & -8.51\% & -3.53\% & -4.45\% & -3.71\% \\
NbrReg & -30.44\% & -15.98\% & -18.84\% & -14.83\% \\
NASH & -9.24\% & -5.58\% & -5.12\% & -4.21\% \\
RBSH & -1.39\% & -1.15\% & -1.55\% & -1.71\% \\
PairRec & -2.40\% & -0.38\% & -0.70\% & -0.29\% \\ \hline
MISH & \textbf{0.00\%} & \textbf{-0.13\%} & \textbf{0.00\%} & \textbf{-0.11\%} \\
    \bottomrule
    \end{tabular}}
    \caption{\cah{Template is acting weird and not showing this table unless it it huge.} Average decrease in worst case and average case prec@100 compared to the best  scores per dataset. An average decrease of 0\% corresponds to obtaining the best performance across all datasets.\label{tab:deltagap}}
\end{table}

==> Unsupervised Multi-Index Semantic Hashing (WWW) (1)/restables.tex <==
\begin{table*}
    \centering
        \caption{Worst case and average case precision@100. The highest precision is highlighted in bold, and the second highest is underlined. $^{\blacktriangle}$ represents statistically significant improvements over the second best method at the 0.05 level using a two tailed paired t-test.}\vspace{-5pt}

    \resizebox{\linewidth}{!}
     {
    \begin{tabular}{l|cc|cc|cc|cc|cc|cc}
    \toprule
         &  \multicolumn{4}{c|}{Reuters} &  \multicolumn{4}{c|}{TMC} &  \multicolumn{4}{c}{Agnews} \\ 
         & \multicolumn{2}{c}{32 bits} & \multicolumn{2}{c|}{64 bits} & \multicolumn{2}{c}{32 bits} & \multicolumn{2}{c|}{64 bits} & \multicolumn{2}{c}{32 bits} & \multicolumn{2}{c}{64 bits} \\
         Prec@100 & Worst & Average & Worst & Average & Worst & Average & Worst & Average & Worst & Average & Worst & Average \\ 
         \midrule
LCH & 0.5995 & 0.6616 & 0.6283 & 0.6613 & 0.6658 & 0.7510 & 0.7421 & 0.7817 & 0.6822 & 0.7599 & 0.7423 & 0.7775\\
STH & 0.7730 & 0.8046 & 0.7803 & 0.7968 & 0.6858 & 0.7693 & 0.7481 & 0.7816 & 0.6823 & 0.8237 & 0.7931 & 0.8374\\
NbrReg & 0.5785 & 0.6329 & 0.6327 & 0.6616 & 0.3272 & 0.6648 & 0.5862 & 0.6827 & 0.7274 & 0.7914 & 0.7535 & 0.7928\\
NASH & 0.7330 & 0.7737 & 0.7767 & 0.7967 & 0.6845 & 0.7709 & 0.7535 & 0.7953 & 0.7059 & 0.8018 & 0.7748 & 0.8107\\
RBSH & 0.7809 & 0.8110 & 0.8011 & 0.8182 & \underline{0.7459} & 0.8107 & 0.7852 & 0.8158 & \underline{0.7797} & 0.8347 & 0.8053 & 0.8317\\
PairRec & \underline{0.7812} & \underline{0.8218} & \underline{0.8087} & \underline{0.8316} & 0.7320 & \textbf{0.8187} & \underline{0.7922} & \textbf{0.8288} & 0.7700 & \underline{0.8348} & \underline{0.8114} & \underline{0.8407}\\ \hline
MISH & \textbf{0.7965} & \textbf{0.8286} & \textbf{0.8248} & \textbf{0.8377} & \textbf{0.7608}$^{\blacktriangle}$ & \underline{0.8156} & \textbf{0.7931} & \underline{0.8261} & \textbf{0.7818} & \textbf{0.8375} & \textbf{0.8116} & \textbf{0.8419}\\
    \bottomrule
    \end{tabular}}
    \label{tab:resultsPerf}
    %\vspace{-10pt}
\end{table*}
\begin{table*}
    \centering
        \caption{Speedup of multi-index hashing over a brute-force linear scan, as well as linear scan time per document. Greedy substring optmizing (GSO) \cite{norouzi2012fast} corresponds to the correlation-based post-hoc heuristic, and Default corresponds to using the hash codes as is. The largest speedup is highlighted in bold (independent of post-hoc fix), and the second largest is underlined. $^{\blacktriangle}$ represents statistically significant improvements  (100 repeated timing experiments) over the second best method at the 0.05 level using a two tailed paired t-test.}\vspace{-5pt}

    \resizebox{\linewidth}{!}
     {
    \begin{tabular}{l|cc|cc|cc|cc|cc|cc}
    \toprule
         &  \multicolumn{4}{c|}{Reuters} &  \multicolumn{4}{c|}{TMC} &  \multicolumn{4}{c}{Agnews} \\ 
         & \multicolumn{2}{c}{32 bits} & \multicolumn{2}{c|}{64 bits} & \multicolumn{2}{c}{32 bits} & \multicolumn{2}{c|}{64 bits} & \multicolumn{2}{c}{32 bits} & \multicolumn{2}{c}{64 bits} \\
         Speedup & Default & GSO & Default & GSO & Default & GSO & Default & GSO & Default & GSO & Default & GSO \\ \midrule
LCH & 2.5182 & 0.3508 & 0.8937 & 0.5603 & 7.2427 & 1.5879 & 2.1837 & 3.0767 & 18.2709 & 25.6365 & 3.7311 & 5.1354\\
STH & 2.9374 & 0.2783 & 1.0116 & 0.5695 & 7.0382 & 2.2211 & 2.1947 & 2.4791 & 14.6936 & 29.2779 & 4.4515 & \underline{9.5676}\\
NbrReg & \underline{6.3841} & 0.7190 & \underline{4.9589} & 0.8299 & 7.1497 & 1.7346 & 2.8800 & \underline{5.2506} & 21.7102 & 23.7698 & 6.8518 & 7.5279\\
NASH & 5.6356 & 0.6037 & 4.5869 & 0.8417 & 9.4069 & 1.5725 & 4.3819 & 4.3886 & 20.7673 & 23.1443 & 4.8355 & 5.3849\\
RBSH & 4.4342 & 0.2965 & 1.7083 & 0.8051 & 7.0831 & 1.9708 & 2.7957 & 2.9146 & 25.9186 & 27.1164 & 4.5036 & 4.7345\\
PairRec & 5.4296 & 0.3721 & 3.0770 & 0.9433 & \underline{10.9118} & 1.7063 & 5.1129 & 4.9614 & 29.7880 & \underline{33.4096} & 7.1765 & 7.8676\\ \hline
MISH & \textbf{7.0698}$^{\blacktriangle}$& 1.1216 & \textbf{5.4466}$^{\blacktriangle}$& 1.0282 & \textbf{14.6296}$^{\blacktriangle}$& 2.1923 & \textbf{8.8696}$^{\blacktriangle}$& 6.1645 & \textbf{44.0151}$^{\blacktriangle}$& 35.9177 & \textbf{13.6756}$^{\blacktriangle}$& 12.5788\\
    \bottomrule
Linear scan time & \multicolumn{2}{c|}{0.000070 s} & \multicolumn{2}{c|}{0.000069 s} & \multicolumn{2}{c|}{0.000111 s} & \multicolumn{2}{c|}{0.000109 s} & \multicolumn{2}{c|}{0.000432 s} & \multicolumn{2}{c|}{0.000407 s} \\ \bottomrule
    \end{tabular}}
    \label{tab:resultsSpeed}
    %\vspace{-10pt}
\end{table*}

==> deltatable.tex <==
\begin{table}
    \centering
    \resizebox{\linewidth}{!}
    {
    \begin{tabular}{l|cc|cc}
    \toprule
    & \multicolumn{2}{c}{32 bits} & \multicolumn{2}{c}{64 bits} \\ 
    & $\Delta$ worst case & $\Delta$ average & $\Delta$ worst case & $\Delta$ average \\ \midrule
LCH & -16.65\% & -12.57\% & -12.93\% & -11.46\% \\
STH & -8.51\% & -3.53\% & -4.45\% & -3.71\% \\
NbrReg & -30.44\% & -15.98\% & -18.84\% & -14.83\% \\
NASH & -9.24\% & -5.58\% & -5.12\% & -4.21\% \\
RBSH & -1.39\% & -1.15\% & -1.55\% & -1.71\% \\
PairRec & -2.40\% & -0.38\% & -0.70\% & -0.29\% \\ \hline
MISH & \textbf{0.00\%} & \textbf{-0.13\%} & \textbf{0.00\%} & \textbf{-0.11\%} \\
    \bottomrule
    \end{tabular}}
    \caption{\cah{Template is acting weird and not showing this table unless it it huge.} Average decrease in worst case and average case prec@100 compared to the best  scores per dataset. An average decrease of 0\% corresponds to obtaining the best performance across all datasets.\label{tab:deltagap}}
\end{table}
